Graph-CoVis: GNN-based Multi-view Panorama Global Pose Estimation

In this paper, we address the problem of wide-baseline camera pose estimation from a group of 360$^\circ$ panoramas under upright-camera assumption. Recent work has demonstrated the merit of deep-learning for end-to-end direct relative pose regression in 360$^\circ$ panorama pairs [11]. To exploit the benefits of multi-view logic in a learning-based framework, we introduce Graph-CoVis, which non-trivially extends CoVisPose [11] from relative two-view to global multi-view spherical camera pose estimation. Graph-CoVis is a novel Graph Neural Network based architecture that jointly learns the co-visible structure and global motion in an end-to-end and fully-supervised approach. Using the ZInD [4] dataset, which features real homes presenting wide-baselines, occlusion, and limited visual overlap, we show that our model performs competitively to state-of-the-art approaches.

==> additional_ATE_plots.tex <==
For the three-view setting, we study the error as a function of distance, rotation, and co-visibility of the panoramas with respect to the origin panorama.
Figure \ref{fig:ate_vs_mean_dist} shows the translation error (ATE) as a function of mean distance of the panoramas from the origin panorama. For easier comparison, the first and second order polynomial fits to the points in the three plots are shown in Figure~\ref{fig:ate_vs_mean_dist_curves}. Graph-Covis consistently out-performs CoVisPose+Greedy and CoVisPose+PGO baselines for all distances from the origin panorama.

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.75\linewidth]{images/ATE_vs_X_plots/1_mean_origin_distance_error.png}
    \caption{Mean distance of panoramas to origin (x axis, meters) v/s ATE (y axis, meters) for CovisPose+Greedy, CovisPose+PGO, and Graph-Covis. The yellow and red curves are first and second order polynomial fits to the data points.} 
    \label{fig:ate_vs_mean_dist}
\end{figure*}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.8\linewidth]{images/ATE_vs_X_plots/1b_mean_origin_distance_interp_curves.png}
    \caption{First (left) and second (right) order polynomial fits to ATE values in Figure \ref{fig:ate_vs_mean_dist} show that Graph-Covis (green solid) consistently outperforms other baselines (dashed).}
    \label{fig:ate_vs_mean_dist_curves}
\end{figure*}


Figure~\ref{fig:ate_vs_mean_rot} shows the translation error (ATE) as a function of mean rotation of the panoramas compared to the origin panorama. Direct comparison of the curves in Figure~\ref{fig:ate_vs_mean_rot_curves} shows Graph-Covis consistently out-performs baselines for all rotation values. %from origin.

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.75\linewidth]{images/ATE_vs_X_plots/4_mean_origin_rotation_error.png}
    \caption{Mean absolute rotation of panoramas to origin (x axis, degrees) v/s ATE (y axis, meters) for CovisPose+Greedy, CovisPose+PGO, and Graph-Covis. The yellow and red curves are first and second order polynomial fits to the data points.} 
    \label{fig:ate_vs_mean_rot}
\end{figure*}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.8\linewidth]{images/ATE_vs_X_plots/4b_mean_origin_rotation_interp_curves.png}
    \caption{First (left) and second (right) order polynomial fits to ATE values in Figure \ref{fig:ate_vs_mean_rot} show that Graph-Covis (green solid) consistently outperforms other baselines (dashed).}
    \label{fig:ate_vs_mean_rot_curves}
\end{figure*}


Finally, Figure~\ref{fig:ate_vs_mean_covis} shows the translation error (ATE) as a function of mean co-visibility of the panoramas compared to the origin panorama. Graph-Covis performs better than baselines for larger co-visibilities. Similar to Section~\ref{sec:generalize_graph_covis}, the distribution of training samples in Figure~\ref{fig:ate_covis_distribution} shows that there are very few training examples with low mean co-visibility. The performance of Graph-Covis may be improved in the lower co-visibility range by adding more training examples in this region.

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.75\linewidth]{images/ATE_vs_X_plots/7_mean_origin_covis_error.png}
    \caption{Mean co-visibility of panoramas to origin (x axis, percentage) v/s ATE (y axis, meters) for CovisPose+Greedy, CovisPose+PGO, and Graph-Covis. The yellow and red curves are first and second order polynomial fits to the data points.} 
    \label{fig:ate_vs_mean_covis}
\end{figure*}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.8\linewidth]{images/ATE_vs_X_plots/7b_mean_origin_covis_interp_curves.png}
    \caption{First (left) and second (right) order polynomial fits to ATE values in Figure \ref{fig:ate_vs_mean_covis} show that Graph-Covis (green solid) outperforms other baselines (dashed) for higher values of co-visibility.}
    \label{fig:ate_vs_mean_covis_curves}
\end{figure*}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=.5\linewidth]{images/ATE_vs_X_plots/7c_mean_origin_covis_density.png}
    \caption{Distribution of samples over different co-visibility values. The worse performance of Graph-CoVis for lower co-visibility examples in Figure \ref{fig:ate_vs_mean_covis_curves} is likely due to the low number of training examples in this region.}
    \label{fig:ate_covis_distribution}
\end{figure*}


==> overview.tex <==
Our Graph-CoVis architecture is shown in Figure \ref{fig:architecture}. Graph-CoVis accepts as input a set of indoor $360^\circ$ panoramas and estimates a 3-DOF pose in a shared coordinate system. The camera is assumed upright at a fixed height for each home (planar camera motion model).
%, which is common in indoor robotics\cite{choi2018fast, Guan_2020_CVPR} and virtual walk-through applications~\cite{aly2012street, Cruz2021ZillowID}.
%The panoramas are straightened to ensure the upright camera axis is oriented with the gravity vector. 
%As in ZInD, we assume Atlanta world layouts, with upright walls that are orthogonal to the floor. 
The architecture is capable of estimating poses for variable size input groups, although we focus on the three-view case in this paper.
%with the maximum number of panoramas being dictated by the GPU memory available at training time. 

Graph-CoVis encodes node and edge feature representations in the graph and refines them through six message passing layers. Message passing between nodes is mediated first by a transformer encoder, which encodes relationships between nodes along the edges, followed by a transformer decoder, which computes node update messages given the neighboring node's embedding as well as the edge embedding. 

% Inspired with CoVis-Pose we extracted rich representations such as angular correspondence, co-visibility, and layout boundary from the final edge representations to help the model understand the geometry. Additionally, as nodes are updating using massages from every nodes and adjacent edges, it has more global information, therefore we estimate the global pose using a 3-layer MLP.

To encourage extraction of rich representations for global pose estimation, as in CoVisPose\cite{Hutchcroft_2022}, we estimate the angular correspondence, visual overlap (co-visibility), and layout boundary from the final edge representations with a single linear layer. Finally, from each node representation, we estimate the global pose using a 3-layer MLP. 
%This structure helps the model even in absence of enough covisibility.\manju{How? Justify or remove claim}

Through our designed message passing scheme, the GNN learns to encode pair-wise geometric cues along the edges, that are then globally aggregated in the node representations, in order to accurately estimate poses for multiple views of an indoor space. 

% Through our designed message passing scheme, the GNN learns to encode high level complex relationships between pose, co-visibility, and structure in visually overlapping parts from mutliple views of an indoor space. The model is able to replicate in principle and improve in accuracy over classical baseline solutions to modeling
% the multi-view relationships.
%\naji{I think it might be a good idea to re-order this section and put more focus on "additions" to the Covis architecture and the value they unlocked. i.e. pointing out Covis architectural limitations, how we addresses those in these additions by talking about GNN and how it made our framework general to number of panos and at the end point out the parts that are shared between covis and graph covis. Reading this section, gave me a feeling of downplaying graph covis by putting a lot of focus on how much it borrowed from covis and not putting enough focus on what's new.}

% So far we have  to estimate the relative pose of two panoramas \ref{}. However, wide range of applications in this are looking for a global camera pose. Estimating the top-down layout of a room from multiple panoramas, reconstructing the 3D representation of the a room, and Simultaneous localisation and Mapping (SLAM) are some of the applications which are crucial for visual perception and understanding. 

% As mentioned earlier, in order to estimate the global pose, previous techniques Consistes of two parts, first, estimating the reletive pose of the pairs, second, defining a global coordinate system  pairwise pose estimation models \ref{super-glue,covis,sift,lofter} to estimate pairwise pose and then. In this work we have presented a novel idea which we 

% The Graph\-Covis architecture is shown in Figure \ref{}. The proposed model input is a set of $360^{\circ}$ panoramas in equirectangular projection, captured in indoor space. The model outputs two sets of information, the pose of each pano in a defined global coordinate system and geometric information such as Co-visibility, angular Correspondence and Floor-wall boundary (CCF). 
